Shrinkage-based random local clocks with scalable inference

Local clock models propose that the rate of molecular evolution is constant within phylogenetic sub-trees. Current local clock inference procedures scale poorly to large taxa problems, impose model misspecification, or require a priori knowledge of the existence and location of clocks. To overcome these challenges, we present an autocorrelated, Bayesian model of heritable clock rate evolution that leverages heavy-tailed priors with mean zero to shrink increments of change between branch-specific clocks. We further develop an efficient Hamiltonian Monte Carlo sampler that exploits closed form gradient computations to scale our model to large trees. Inference under our shrinkage-clock exhibits an over 3-fold speed increase compared to the popular random local clock when estimating branch-specific clock rates on a simulated dataset. We further show our shrinkage-clock recovers known local clocks within a rodent and mammalian phylogeny. Finally, in a problem that once appeared computationally impractical, we investigate the heritable clock structure of various surface glycoproteins of influenza A virus in the absence of prior knowledge about clock placement.

==> mathMacros.tex <==
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{hyperref}

\usepackage{graphicx} % support the \includegraphics command and options
%\usepackage{setspace}

% \usepackage[parfill]{parskip} % Activate to begin paragraphs with an empty line rather than an indent

%%% PACKAGES
% \usepackage{booktabs} % for much better looking tables
\usepackage{array} % for better arrays (eg matrices) in maths
\usepackage{paralist} % very flexible & customisable lists (eg. enumerate/itemize, etc.)
\usepackage{verbatim} % adds environment for commenting out blocks of text & for better verbatim
\usepackage{subfig} % make it possible to include more than one captioned figure/table in a single float
\usepackage{amsbsy}
\usepackage{amsmath}
% \usepackage{bbold}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amscd}
\usepackage{amsthm}
\usepackage{cite}
\usepackage{float}
% \usepackage[toc,page]{appendix}
\usepackage{natbib}
% \usepackage{lineno}
\usepackage{mathrsfs}
\usepackage{bbm}
% \usepackage[nolists]{endfloat}
% ^ puts graphs at end of doc.
% \usepackage{lineno}
% \usepackage{todonotes}
% \usepackage{setspace}
% \usepackage{multirow}


\def\diffvar{\boldsymbol{\Sigma}}

\newcommand{\slab}{\xi}
\newcommand{\cDensity}[2]{\ensuremath{p(#1 \,|\,#2)}}
\newcommand{\density}[1]{\ensuremath{p(#1 )}}
\newcommand{\vecOperator}[1]{\mbox{vec}\hspace{-0.1em}\left[ #1 \right]}
\newcommand{\trOperator}[1]{\mbox{tr}\hspace{-0.1em}\left[ #1 \right]}
\newcommand{\oneVector}[1]{\mathbf{1}_{#1}}
\newcommand{\order}[1]{{\mathcal O}\hspace{-0.1em}\left( #1 \right)}
\newcommand{\specialInverse}{^-}
\newcommand{\inverse}{^{-1}}
\newcommand{\transpose}{^t}
\newcommand{\vectorize}[1]{\text{vec}\left(#1\right)}
\newcommand{\kronecker}{\otimes}

\newcommand{\position}{\mathbf{q}}
\newcommand{\allMomentum}{\boldsymbol{\nu}}
\newcommand{\momentumi}{\rho_i}

\newcommand{\rootTraitMean}{\boldsymbol{\nu}_0}
\newcommand{\rootSampleSize}{\kappa_0}
\newcommand{\parent}[1]{\text{pa}(#1)}
\newcommand{\sister}[1]{\text{sis}(#1)}
\newcommand{\smallParent}[1]{\text{\tiny pa}(#1)}
\newcommand{\nodePrecision}[1]{\mathbf{P}_{#1}}
\newcommand{\nodeVariance}[1]{\mathbf{\mathbf{V}}_{#1}}
\newcommand{\nodeVarianceFunction}[1]{\nodeVariance{}\hspace{-0.25em}\left( #1 \right)}
\newcommand{\paramList}{\boldsymbol{\theta}}

\newcommand{\general}[1]{g{}\hspace{-0.1em}\left( #1 \right)}

\newcommand{\vY}{\mathbf{y}}
\newcommand{\vP}{\mathbf{P}}
\newcommand{\vL}{\mathbf{L}}

\newcommand{\deflatedNodePrecision}[1]{\nodePrecision{#1}^{\star}}
\newcommand{\nodeMean}[1]{\mathbf{m}_{#1}}
\newcommand{\nodeIndexOne}{i}
\newcommand{\nodeIndexTwo}{j}
\newcommand{\nodeIndexThree}{k}
\newcommand{\branchLength}[1]{t_{#1}}
\newcommand{\diffusionVariance}{\diffvar}
\newcommand{\remainder}[1]{r_{#1}}
\newcommand{\backback}{-0.15em}
\newcommand{\zeroDimension}[1]{d\hspace{\backback}\left(#1\right)}
\newcommand{\infiniteDimension}[1]{e\hspace{\backback}\left(#1\right)}
\newcommand{\finiteNonZeroDimension}[1]{f\hspace{\backback}\left(#1\right)}
\newcommand{\permutationMatrix}{\mathbf{Q}}
\newcommand{\nodePermutationMatrix}[1]{\permutationMatrix_{#1}}
\newcommand{\missing}[2]{\delta_{#1 #2}}
\newcommand{\traitIndex}{p}
\newcommand{\arbitraryMatrix}{\mathbf{Z}}
\newcommand{\identityMatrix}[1]{\mathbf{I}_{#1}}
\newcommand{\bigzero}[2]{\makebox(0,0){\hspace{#1}\vspace{#2}\text{\huge0}}}
\newcommand{\altDet}[1]{\hat{\text{det}}\left( #1 \right)}
\newcommand{\changeDimension}[1]{\Delta_{#1}}
\newcommand{\notMissingMatrix}[1]{\boldsymbol{\delta}_{#1}}

\newcommand{\nodePreMean}[1]{\mathbf{n}_{#1}}
\newcommand{\nodePreVariance}[1]{\mathbf{W}_{#1}}
\newcommand{\nodePrePrecision}[1]{\mathbf{Q}_{#1}}
\newcommand{\deflatedNodePrePrecision}[1]{\nodePrePrecision{#1}^{\star}}
\newcommand{\Indexobs}{\mathcal{I}^{\text{\tiny obs}}_ \nodeIndexOne}
\newcommand{\Indexmis}{\mathcal{I}^{\text{\tiny mis}}_ \nodeIndexOne}

\newcommand{\normalDensityFunction}[3]{{\mathcal N}\hspace{-0.25em}\left( #1; #2, #3 \right)}
\newcommand{\normalDensity}[2]{{\mathcal N}\hspace{-0.25em}\left( #1, #2 \right)}
\newcommand{\normalVariance}{\sigma^2}
\newcommand{\conditionalMean}[1]{\boldsymbol{\mu}_{#1}}
\newcommand{\dd}{\text{d}}
\def\rowvarresidMissing{\rowvarresid_{{mis}_\nodeIndexOne}}

\newcommand{\momentum}[1]{\nu_{#1}}
\newcommand{\branchRateSD}{s}
\newcommand{\symbolicObservedVariance}{0}
\newcommand{\symbolicMissingVariance}{\infty}
\newcommand{\symbolicFiniteVariance}{+}
\newcommand{\partialDiffusionVariance}[2]{\diffusionVariance_{#1 #2}}
\newcommand{\observedMatrix}[1]{\boldsymbol{\delta}_{#1}}

\newcommand{\observedVariance}{\partialDiffusionVariance{\symbolicObservedVariance}{\symbolicObservedVariance}}
\newcommand{\missingVariance}{\partialDiffusionVariance{\symbolicMissingVariance}{\symbolicMissingVariance}}
\newcommand{\finiteVariance}{\partialDiffusionVariance{\symbolicFiniteVariance}{\symbolicFiniteVariance}}
\newcommand{\tipLatentPrecision}[1]{\mathbf{R}_{#1}}

\newcommand{\massMatrix}{\mathbf{M}}
\newcommand{\Hessian}{\mathcal{H}}
\newcommand{\finiteObservedVariance}{\partialDiffusionVariance{\symbolicFiniteVariance}{\symbolicObservedVariance}}
\newcommand{\finiteMissingVariance}{\partialDiffusionVariance{\symbolicFiniteVariance}{\symbolicMissingVariance}}
\newcommand{\observedMissingVariance}{\partialDiffusionVariance{\symbolicObservedVariance}{\symbolicMissingVariance}}
\newcommand{\diag}[1]{\text{diag} \left[ #1 \right]}

\newcommand{\deflatedPrecision}[1]{\mathbf{P}^{\star}_{#1}}
\newcommand{\startingPrecision}[1]{\mathbf{P}_{#1}}
\newcommand{\finitePrecision}[1]{\tilde{\startingPrecision{#1}}}
\newcommand{\bogusPrecision}[1]{\finitePrecision{#1}^{-1}}
\newcommand{\raisedInfty}{\raisebox{0.1em}{$\infty$}}
\newcommand{\bfZero}{\mathbf{0}}
\newcommand{\missingIndicator}[1]{\mathbf{M}_{#1}}
\newcommand{\indicator}{\delta}
\newcommand{\indicatorFunction}{\mathbbm{1}}
\newcommand{\phylogeny}{\mathscr{F}}
\newcommand{\phylogenyVariance}{\mathbf{\Upsilon}}
\newcommand{\phylogenyPrecision}{\phylogenyVariance\inverse}
\newcommand{\traitPrecision}{\mathbf{P}}

\newcommand{\grandVariance}{\mathbf{\Sigma}}
\newcommand{\grandVarianceExpression}{\traitPrecision\inverse \kronecker \phylogenyVariance}
\newcommand{\grandPrecision}{\grandVariance\inverse}
\newcommand{\grandPrecisionExpression}{\traitPrecision \kronecker \phylogenyPrecision}

\newcommand{\latentData}{\mathbf{Y}}
\newcommand{\vecLatentData}{\mathbf{Z}}
\newcommand{\nTaxa}{N}
\newcommand{\nTraits}{P}
\newcommand{\latentObs}[1]{\latentData_{#1}^{\{ \text{o} \}}}
\newcommand{\latentUnobs}[1]{\latentData_{#1}^{\{ \text{u} \}}}
\newcommand{\obs}{^{ \text{o} }}
\newcommand{\unobs}{^{\text{u}}}
\newcommand{\obsUnobs}{^{\text{uo}}}
\newcommand{\mvnDensity}[2]{\text{MVN}\hspace{-0.1em}\left(#1, #2\right)}
\newcommand{\mvn}[3]{\text{MVN}\hspace{-0.1em}\left(#1; #2, #3\right)}
\newcommand{\gradient}[1]{\frac{\partial}{\partial #1}}
\newcommand{\gradientTwo}[2]{\frac{\partial^2}{\partial #1 \partial #2}}

\newcommand{\transformMatrix}{\mathbf{T}}
\newcommand{\condensedLikelihood}{L\hspace{-0.2em}\left[\allScaledRates\left(\allRates\right)\right]}
\newcommand{\fullGradient}[1]{\nabla_{#1}}
\newcommand{\gradEz}{\frac{\partial}{\partial \phi_i}}
\newcommand{\gradTwoEz}{\frac{\partial^2}{\partial \phi_i^2}}
\newcommand{\functionG}{\mathbf{G}(\mathbf{Y}_i)}

\newcommand{\sequence}{\mathbf{S}}
\newcommand{\priorVariance}{\mathbf{V}}
\newcommand{\rate}[1]{r_{#1}}
\newcommand{\scaledRate}[1]{\rho_{#1}}
\newcommand{\allRates}{\mathbf{r}}
\newcommand{\allScaledRates}{\boldsymbol{\rho}}
\newcommand{\var}[1]{\mathbb{V}\hspace{-0.1em}\left[ #1 \right]}
\newcommand{\drift}[1]{\boldsymbol{\mu}_{#1}}
%
\newcommand{\fullConditionalMean}[1]{\boldsymbol{\mu}_{#1}}
\newcommand{\fullConditionalVariance}[1]{\mathbf{Z}_{#1}}
%
\newcommand{\below}[1]{\lfloor #1 \rfloor}
\renewcommand{\above}[1]{\lceil #1 \rceil}
\newcommand{\expectation}[1]{\mathbb{E}\hspace{-0.1em}\left[ #1 \right]}
\newcommand{\nodePostVariance}[1]{\mathbf{R}_{#1}}
\newcommand{\jointPairData}[1]{\mathbf{Z}_{#1}}
\newcommand{\jointPairDataExpression}{
\left( \begin{array}{l}
\latentData_{\nodeIndexOne} \\
\latentData_{\parent{\nodeIndexOne}}
\end{array}
\right)
}
\newcommand{\transformedJointPairData}{\mathbf{X}}
\newcommand{\cholesky}[1]{\mathbf{L}_{#1}}
\newcommand{\linearTransformExpression}{
\left( \begin{array}{rr}
	1 & -1 \\
	1 &  1
\end{array} \right)
}
\newcommand{\linearTransform}{\mathbf{A}}

\def\treeTraitsRoot{\boldsymbol{\mu}_R}
\def\diffprec{\boldsymbol{\Lambda}_R}
\def\diffprecprior{\boldsymbol{\Lambda}_{R_0}}
\def\diffmean{\boldsymbol{\mu}_0}
\def\pss{\kappa_0}
\def\diffprecpriordf{\nu}
\def\pss{\kappa_0}

\newcommand{\functional}[1]{\mathbf{F}\hspace{-0.1em}\left( #1 \right)}
\newcommand{\nastyPrecision}[1]{\boldsymbol{\Upsilon}_{#1}}
\newcommand{\nastyDeterminant}[1]{\boldsymbol{\chi}_{#1}}

%% shrinkage paper
% \newcommand{\phylogeny}{\mathscr{F}}
% \newcommand{\rate}[1]{r_{#1}}
% \newcommand{\allRates}{\mathbf{r}}
% \newcommand{\nodeIndexOne}{i}
% \newcommand{\nodeIndexTwo}{j}
% \newcommand{\nodeIndexThree}{k}
\newcommand{\nIndex}{n}
\newcommand{\traitData}{\mathbf{Y}}
\newcommand{\sequenceData}{\mathbf{S}}
% \newcommand{\parent}[1]{\text{pa}(#1)}
% \newcommand{\branchLength}[1]{t_{#1}}
\newcommand{\branch}[1]{b_{#1}}
% \newcommand{\mvnDensity}[2]{\text{MVN}\hspace{-0.1em}\left(#1, #2\right)}
\newcommand{\nDensity}[2]{\text{N}\hspace{-0.1em}\left(#1, #2\right)}
% \newcommand{\diffusionVariance}{\boldsymbol{\Sigma}}
\newcommand{\nSequence}{N}
\newcommand{\rateMatrix}{\mathbf{Q}}
% \newcommand{\nTaxa}{N}

% \newcommand{\cDensity}[2]{\ensuremath{p(#1 \,|\,#2)}}
% \newcommand{\density}[1]{\ensuremath{p(#1 )}}
% \newcommand{\vecOperator}[1]{\mbox{vec}\left[ #1 \right]}
% \newcommand{\trOperator}[1]{\mbox{tr}\left[ #1 \right]}
% \newcommand{\oneVector}[1]{\mathbf{1}_{#1}}
% \newcommand{\order}[1]{{\cal O} \left( #1 \right)}
% \newcommand{\specialInverse}{-}
% \newcommand{\inverse}{^{-1}}
\newcommand{\transitionMatrix}{\mathbf{P}}
% \newcommand{\nodeVariance}[1]{\mathbf{\mathbf{V}}_{#1}}
% \newcommand{\nodeVarianceFunction}[1]{\nodeVariance{}\hspace{-0.25em}\left( #1 \right)}

% \newcommand{\paramList}{\boldsymbol{\theta}}
\newcommand{\localVar}[1]{\lambda_{#1}}
\newcommand{\allLocalVar}{\boldsymbol{\lambda}}
\newcommand{\globalVar}{\mu}
\newcommand{\increment}[1]{\phi_{#1}}
\newcommand{\allIncrements}{\boldsymbol{\phi}}
 \newcommand{\exponential}[1]{\text{exp}\{{#1}\}}
%  \newcommand{\gradient}[1]{\frac{\partial}{\partial #1}}
 \newcommand{\rateTransform}{M}
 \newcommand{\logRate}[1]{c_{#1}}
 \newcommand{\logAllRates}{\mathbf{c}}
 \newcommand{\relevantData}{\mathbf{X}}
 \newcommand{\relevantParameters}{\boldsymbol{\theta}}
 \newcommand{\incrementFunction}{g \left( \sum_{\nodeIndexOne} \increment{\nodeIndexOne} \right)}
 \newcommand{\rateVariation}{s_\siteIndex}
% \graphicspath{{../figures/}}

\newcommand{\location}{\gamma}
\newcommand{\exponent}{\alpha}
\newcommand{\incDistribution}{P_{\allIncrements}}
\newcommand{\iidSim}{\stackrel{\tiny\mbox{iid}}{\sim}}
\newcommand{\numDes}[1]{d_{#1}}
\newcommand{\incrementPrior}{\cDensity{\allIncrements}{\allLocalVar, \globalVar}}
\newcommand{\ratesPrior}{\cDensity{\allRates}{\allLocalVar, \globalVar}}

\newcommand{\bridgeVariance}[1]{\sigma_{#1}^2}
\newcommand{\fullBridgePrecision}[1]{\left(\frac{1}{\slab^2} + \frac{1}{\localVar{#1}^2 \globalVar^2} \right)}
\newcommand{\fullBridgeVariance}[1]{\fullBridgePrecision \inverse}


% figure
% \frac{d {\boldsymbol{\phi}}}{d \mathbf{r}} = \begin{bmatrix}
%     \frac{1}{r_1} & 0 & 0 & 0 & \llap{-} \frac{1}{r_5} & 0\\[.2cm]
% 0 & \frac{1}{r_2} & 0 & 0 & \llap{-} \frac{1}{r_5} & 0\\[.2cm]
% 0 & 0 & \frac{1}{r_3} & 0 & 0 & \llap{-} \frac{1}{r_6}\\[.2cm]
% 0 & 0 & 0 & \frac{1}{r_4} & 0 & 0\\[.2cm]
% 0 & 0 & 0 & 0 & \frac{1}{r_5} & \llap{-} \frac{1}{r_6}\\[.2cm]
% 0 & 0 & 0 & 0 & 0 & \frac{1}{r_6}
%   \end{bmatrix}

